Guarantees for Real Robotic Systems: Unifying Formal Controller Synthesis and Reachset-Conformant Identification

Robots are used increasingly often in safety-critical scenarios, such as robotic surgery or human-robot interaction. To ensure stringent performance criteria, formal controller synthesis is a promising direction to guarantee that robots behave as desired. However, formally ensured properties only transfer to the real robot when the model is appropriate. We address this problem by combining the identification of a reachset-conformant model with controller synthesis. Since the reachset-conformant model contains all the measured behaviors of the real robot, the safety properties of the model transfer to the real robot. The transferability is demonstrated by experiments on a real robot, for which we synthesize tracking controllers.

==> sections/ProblemStatement.tex <==
% !TEX root = ../TRO2021.tex
\section{Problem Statement}\label{sec_preliminaries}

